Label-Only Model Inversion Attacks via Knowledge Transfer

In a model inversion (MI) attack, an adversary abuses access to a machine learning (ML) model to infer and reconstruct private training data. Remarkable progress has been made in the white-box and black-box setups, where the adversary has access to the complete model or the model's soft output respectively. However, there is very limited study in the most challenging but practically important setup: Label-only MI attacks, where the adversary only has access to the model's predicted label (hard label) without confidence scores nor any other model information. In this work, we propose LOKT, a novel approach for label-only MI attacks. Our idea is based on transfer of knowledge from the opaque target model to surrogate models. Subsequently, using these surrogate models, our approach can harness advanced white-box attacks. We propose knowledge transfer based on generative modelling, and introduce a new model, Target model-assisted ACGAN (T-ACGAN), for effective knowledge transfer. Our method casts the challenging label-only MI into the more tractable white-box setup. We provide analysis to support that surrogate models based on our approach serve as effective proxies for the target model for MI. Our experiments show that our method significantly outperforms existing SOTA Label-only MI attack by more than 15% across all MI benchmarks. Furthermore, our method compares favorably in terms of query budget. Our study highlights rising privacy threats for ML models even when minimal information (i.e., hard labels) is exposed. Our study highlights rising privacy threats for ML models even when minimal information (i.e., hard labels) is exposed. Our code, demo, models and reconstructed data are available at our project page: https://ngoc-nguyen-0.github.io/lokt/

==> sections/checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newpage
\section*{Checklist}

\subsection{TLDR}
"Too Long; Didn't Read": a short sentence describing your paper

{\color{blue}
Our method for label-only model inversion attacks utilizes knowledge transfer from an opaque target model to surrogate models, improving performance compared to SOTA attacks and highlighting privacy threats to ML models with only hard labels exposed.

(maximum 250 characters)

% We propose a 
% new approach for label-only model inversion attacks by using knowledge transfer from a opaque target model to surrogate models, resulting in improved performance compared to existing SOTA attacks, demonstrating the potential privacy threats to ML models even when only hard labels are exposed.
}

\subsection{*Corresponding Author}

Select which author should be the primary corresponding author for this submission. Please enter an email address or an OpenReview ID that exactly matches one of the authors.

{\color{blue}
ngaiman\_cheung@sutd.edu.sg


}


\subsection{*Financial Support}

Optionally indicate one student author on the paper who would need financial support to attend and present at the conference if the paper is accepted (or leave blank if financial support is not needed). Please enter an email address or an OpenReview ID that exactly matches one of the authors.

{\color{blue}

}

\subsection{*Reviewer Nomination}

Please nominate one author who would be willing to review NeurIPS 2023 papers. Receiving these nominations is important for us to ensure that we have enough capable reviewers to review all submissions. Reviewers are expected to have at least two papers in top peer-reviewed conferences or journals, with at least one paper in a machine learning venue (e.g., NeurIPS, ICML, or ICLR) in the last three years, though we still ask that you nominate one of the authors even if none meet this requirement. Please enter an email address or an OpenReview ID that exactly matches one of the authors.

{\color{blue}

ngaiman\_cheung@sutd.edu.sg

}
\subsection{*Primary Area}


Machine vision

Natural Language Processing

Speech and Audio

Deep learning architectures

Generative models

Diffusion based models

Optimization for deep networks

Evaluation (methodology, meta studies, replicability and validity)

Online learning

Bandits

Reinforcement learning

Active learning

Infrastructure (libraries, improved implementation and scalability, distributed solutions)

Machine learning for healthcare

Machine learning for physical sciences (for example: climate, physics)

Machine learning for social sciences

Machine learning for other sciences and fields

Graph neural networks

Neuroscience and cognitive science (neural coding, brain-computer interfaces)

Optimization (convex and non-convex, discrete, stochastic, robust)

Probabilistic methods (for example: variational inference, Gaussian processes)

Causal inference

Robotics

Interpretability and Explainability

Fairness

Privacy

Safety in Machine Learning

Human-AI Interaction

Learning Theory

Algorithmic game theory

Other (please use sparingly, only use the keyword field for more details)


-------------------------------
{\color{blue}
Privacy
}

\subsection{*Claims}

Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? Claims in the paper should match theoretical and experimental results in terms of how much the results can be expected to generalize. The paper's contributions should be clearly stated in the abstract and introduction, along with any important assumptions and limitations. It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. Enter yes, no, or an explanation if appropriate. Answers are visible to reviewers.


{\color{blue}
yes
}


\subsection{*Code Of Ethics}

Have you read the NeurIPS Code of Ethics (https://neurips.cc/public/EthicsGuidelines) and ensured that your research conforms to it? Enter yes, no, or an explanation if appropriate. Answers are visible to reviewers.


{\color{blue}

Yes

}


\subsection{*Broader Impacts}

If appropriate for the scope and focus of your paper, did you discuss potential negative societal impacts of your work? Please see the Paper Checklist Guidelines for detailed instructions and examples of points that you may choose to discuss. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}
yes
}


\subsection{*Limitations}

Did you describe the limitations of your work? You are encouraged to create a separate Limitations section in your paper. Please see the Paper Checklist Guidelines for detailed instructions (https://neurips.cc/public/guides/PaperChecklist). Enter yes, no, or an explanation if appropriate. Answers are visible to reviewers.


{\color{blue}
yes
}

\subsection{*Theory}

If you are including theoretical results, did you state the full set of assumptions of all theoretical results, and did you include complete proofs of all theoretical results? All assumptions should be clearly stated or referenced in the statement of any theorems. The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, authors are encouraged to provide a short proof sketch to provide intuition. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.


{\color{blue}
no
}


\subsection{*Experiments}

If you ran experiments, did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? Please see the NeurIPS code and data submission guidelines for more details. While we encourage release of code and data, we understand that this might not be possible, so no is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark). At submission time, to preserve anonymity, remember to release anonymized versions. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}
Yes
}

\subsection{*Training Details}

If you ran experiments, did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)? The full details can be provided with the code, but the important details should be in the main paper, and information about how hyperparameters were selected should appear either in the paper or supplementary materials. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}

Yes

}

\subsection{*Error Bars}

If you ran experiments, did you report error bars (e.g., with respect to the random seed after running experiments multiple times), or other information about the statistical significance of your experiments? Answer yes if you report error bars, confidence intervals, or statistical significance tests for your main experiments. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}

yes, we report the error bars in the supplementary.
}

\subsection{*Compute}

Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? Ideally, you would provide the compute required for each of the individual experimental runs as well as the total compute. Note that your full research project might have required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}

yes, we report the compute in the supplementary.


}

\subsection{*Reproducibility}

If the contribution is a dataset or model, what steps did you take to make your results reproducible or verifiable? Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), release of a model checkpoint, or other means that are appropriate to your research. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}

yes, our code, pre-trained models, demo and inverted data are included in Supplementary.

}

\subsection{*Safeguards}

Do you have safeguards in place for responsible release of models with a high risk for misuse (e.g., pretrained language models)? Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}
n/a
}

\subsection{*Licenses}

If you are using existing assets (e.g., code, data, models), did you cite the creators and respect the license and terms of use? Cite the original paper that produced the code package or dataset. If possible, include a URL. Be sure to check the original license and respect its conditions. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}

Yes

}

\subsection{*Assets}

If you are releasing new assets, did you document them and provide these details alongside the assets? Researchers should communicate the details of the dataset or the model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}
n/a

}

\subsection{*Human Subjects}

If you used crowdsourcing or conducted research with human subjects, did you include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper. According to the NeurIPS Code of Ethics, you must pay workers involved in data collection, curation, or other labor at least the minimum wage in your country. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}
n/a
}

\subsection{*IRB Approvals}

Did you describe any potential participant risks and obtain Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your institution), if applicable? Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. For initial submissions, do not include any information that would break anonymity, such as the institution conducting the review. Enter yes, no, n/a, or an explanation if appropriate. Answers are visible to reviewers.

{\color{blue}
n/a
}

